Knowledgeable Reader: Enhancing Cloze-Style Reading Comprehension with External Commonsense Knowledge

We introduce a neural reading comprehension model that integrates external commonsense knowledge, encoded as a key-value memory, in a cloze-style setting. Instead of relying only on document-to-question interaction or discrete features as in prior work, our model attends to relevant external knowledge and combines this knowledge with the context representation before inferring the answer. This allows the model to attract and imply knowledge from an external knowledge source that is not explicitly stated in the text, but that is relevant for inferring the answer. Our model improves results over a very strong baseline on a hard Common Nouns dataset, making it a strong competitor of much more complex models. By including knowledge explicitly, our model can also provide evidence about the background knowledge used in the RC process.

==> acknowledgements.tex <==
\subsubsection*{Acknowledgments}
This work is supported by the German Research Foundation as part of the Research Training Group ``Adaptive Preparation of Information from Heterogeneous Sources'' (AIPHES) under grant 
No. GRK 1994/1. 

==> figs/fig-visual-example.tex <==
\begin{figure}[!ht]
 \centering
%\hspace{-0.03\textwidth}
%10 percent%
\minipage{0.42\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figs/2018-02-22-stat-reversed-results-f50.pdf}
  %\caption{10 percent}
  %\label{figure:data-size-per-10}
\endminipage\hfill
\caption{Answer scores for the interactions between combination of \textit{Q_{ctx(+kn)}} and \textit{D_{ctx(+kn)}}.}
\label{figure:stat-reverse-pred}
\vspace*{-4mm}
\end{figure}

==> tables/results-know-ablations-f100.tex <==
\begin{table}[ht!]
\centering
\scalebox{0.78}{
\begin{tabular}{@{}lcccc@{}}
                        & \multicolumn{2}{c}{\textbf{NE}} & \multicolumn{2}{c}{\textbf{CN}} \\
\textbf{$ D_{repr}$ to $Q_{repr}$ interaction}    & \textbf{Dev}         & \textbf{Test}        & \textbf{Dev}        & \textbf{Test}       \\ \hline
$ D_{ctx}$, $Q_{ctx}$ (w/o know)            & 75.50              & 70.30              & 68.20             & 64.80            \\ \hline
$ D_{ctx+kn}$, $Q_{ctx+kn}$   & 75.50           & 70.28          & 69.80           & 65.60           \\
$ D_{ctx}$, $Q_{ctx+kn}$       & 74.20            & 69.88          & 70.40           & 66.56         \\
$ D_{ctx+kn}$, $Q$         & \textbf{77.40  }          & 71.40            & 70.95         & 67.52         \\ \hline
All                     & 76.65          & \textbf{71.52  }        & 70.80           & 67.08         \\ \hline
w/o $ D_{ctx}$, $Q_{ctx}$        & 76.70            & 70.68          & \textbf{71.10  }         & \textbf{67.68  }       \\
w/o $ D_{ctx+kn}$, $Q_{ctx+kn}$ & 76.35          & 70.88          & 70.95         & 67.44         \\
w/o $ D_{ctx}$, $Q_{ctx+kn}$     & 76.90            & 71.32          & 70.70           & 67.12         \\
w/o $ D_{ctx + kn}$, $Q$       & 76.50              & 70.64          & 70.75         & 66.88         \\ \hline
\end{tabular}
}
\caption{Results for different combinations of
interactions between  document (D) and question (Q) \textit{context (ctx)} and \textit{context + knowledge (ctx+kn)} representations. (Subj/Obj, 100 facts)
\label{table:results-know-ablations}
\vspace{-2mm}
\end{table}

